Leveraging Public Data for Practical Private Query Release

In many statistical problems, incorporating priors can significantly improve performance. However, the use of prior knowledge in differentially private query release has remained underexplored, despite such priors commonly being available in the form of public datasets, such as previous US Census releases. With the goal of releasing statistics about a private dataset, we present PMW^Pub, which -- unlike existing baselines -- leverages public data drawn from a related distribution as prior information. We provide a theoretical analysis and an empirical evaluation on the American Community Survey (ACS) and ADULT datasets, which shows that our method outperforms state-of-the-art methods. Furthermore, PMW^Pub scales well to high-dimensional data domains, where running many existing methods would be computationally infeasible.

==> docs/fem_mwem_experiments.tex <==
\section{Two Phase Algorithm without Public Data}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\columnwidth]{images_fem_mwem/adult/fem_mwem_25.png}
%     \caption{The x-axis is the epsilon budget split  between FEM and MWEM. That is: (1) first we run FEM with $\varepsilon$ (2) then we use FEM’s output as the support and initial distribution for MWEM. (3) Finally we run MWEM with privacy $0.5-\varepsilon$ (4) Combined they satisfy $0.5$-DP.
%     }
%     \label{fig:my_label}
% \end{figure}

In this section we consider a two-phase approach that does not require public data. In the first phase, we use part of the privacy budget to generate a synthetic data that can be used as the support of \mwem.


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.95\columnwidth]{images_no_public/adult/fem_mwem_25.png}
    \qquad
    \includegraphics[width=0.95\columnwidth]{images_no_public/adult/fem_mwem_50.png}
    \caption{Showing the error of FEM+MWEM for different privacy budget splits. The blue line shows the error of FEM alone with privacy set to $\varepsilon_0$. The orange and green line give the error of FEM+MWEM for $\varepsilon=0.5$ and $\varepsilon=1$ respectively. The error plot is an average over 5 runs.}
    \label{fig:femmwem}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\columnwidth]{images_no_public/adult/dq_mwem.png}
    \caption{Showing the error of DQ+MWEM for different privacy budget splits. The blue line shows the error of FEM alone with privacy set to $\varepsilon_0$. The orange and green line give the error of DQ+MWEM for $\varepsilon=0.5$ and $\varepsilon=1$ respectively. The error plot is an average over 5 runs.}
    \label{fig:femmwem}
\end{figure}


==> docs/support_analysis.tex <==
\section{Support Analysis}

We can argue that a good support $S\subseteq \cX$ for answering a set of queries $Q$ (with $m$ queries) on a dataset $D$ should be able to satisfy the following equation:


\begin{align} \label{eq:span}
\forall a\in [0,1]^{(m+1) } \exists p\in \Delta(S)
\text{s.t. }
a = M(Q,S) p
\end{align}

Let $s=|S|$. To 
The term $M(Q,S)$ is a $((m+1)\times s)$ matrix where the last row is all ones and the remaining $m$ rows are defined by the answer of the $m$ queries on the support $S$.  If we enumerate elements in $S$ as $\{ x_1,\ldots, x_s \}$ and elements in $Q$ as $\{ q_1,\ldots, q_m \}$ then $M(Q,S)(i,j)=q_i(x_j)$. Thus, we can write equation \cref{eq:span} as 

\begin{align}\label{eq:spanmatrixfrom}
\begin{bmatrix}
a_1, \\  \vdots \\ a_{m+1}
\end{bmatrix}
=
\begin{bmatrix}
q_1(x_1) & \ldots & q_1(x_s) \\ 
\vdots & \ddots & \vdots \\
q_m(x_1) & \ldots & q_(x_s) \\ 
1 & \ldots, & 1 \\ 
\end{bmatrix}
\begin{bmatrix}
p_1, \\  \vdots \\ p_{s}
\end{bmatrix}
\end{align}

The 

The quantifier $a$, represents all possible answers 



Our experiments show that taking a sample from the true population provides a better support for \mwem than generating a random support. 


==> docs/theory.tex <==
\input{math_commands}

\section{Theoretical Analysis}\label{sec:theory}

In this section, we analyze the accuracy of \ours under the assumption that the public and private dataset are i.i.d. samples from two different distributions.
The support of the a dataset $X\in\cX^*$ is the set $\supp(X)=\{x \in \cX : x \in X \}$, and we denote the support of the public dataset $\Dhat $ by $\Xhat = \supp(\Dhat)$. Recall that \ours\ (Algorithm \ref{alg:framework}) takes as input a public dataset and then updates its distribution over the public dataset's support using the same procedure found in \mwem.  We show that the accuracy of \ours\ will depend on the best mixture error over the public dataset support $\Dsupp$, which we characterize using the best mixture error function $\errorLBfunc_{\Dtil,\cQ}:2^\cX\rightarrow [0,1]$ that measures
a given support's ability to approximate the private dataset  $\Dtil$ over the set of queries $\cQ$. 
% The function $\errorLBfunc_{\Dtil,\cQ}$ maps a support $S$ to the best mixture error over the support $S$ to approximate $\Dtil$ over queries $\cQ$. 
The precise definition is as follows: 
%
\begin{definition}
For any support  $S\in 2^\cX$, the best mixture error of $S$ to approximate a dataset $D$ over the queries $Q$ is given by the function:
%
\begin{align*}
    % \besterror = 
    \errorLBfunc_{D,Q}(S)=
    \min_{\mu \in \Delta(S)} 
    \max_{q\in Q}
    \left|
    q\pp{D} - 
    \sum_{x \in S} \mu_x  q(x)
    \right|
\end{align*}
where $\mu \in \Delta(S)$ is a distribution over the set $S$ with $\mu_x \ge 0$ for all $x\in S$ and $\sum_{x\in S} \mu_x = 1$.
\end{definition}
%
Intuitively, \ours\ reweights the public dataset in a differentially private manner to approximately match the private dataset's answers; the function $f_{\Dtil, \cQ}(\Xhat)$ captures how well the best possible reweighting on $\Xhat$ would do in the absence of any privacy constraints. While running \ours does not explicitly require calculating the best mixture error, in practice it may prove useful to release it in a privacy-preserving way. We present the following lemma, which shows that $f_{\Dtil, \cQ}(\Xhat)$ has bounded sensitivity.

\begin{lemma}
For any  support $S\in 2^\cX$ and set $Q$, 
the  best mixture error function $f_{D,Q}$ is $\tfrac{1}{n}$ sensitive. 
That is for any pair of neighboring datasets $D,D'$ of size $n$, $\abs{f_{D,Q}(S)  - f_{D',Q}(S)} \leq \tfrac{1}{n}$.
\end{lemma}

It follows that we can release $f_{\Dtil, \cQ}(\Xhat)$, using the Laplace or Gaussian mechanism with magnitude scaled by $\tfrac{1}{n}$.

We show that, if the public and private datasets are drawn from similar distributions, then, with high probability, $f_{\Dtil, \cQ}(\Xhat)$ is small. Note that the required size of the public dataset increases with the divergence between the private and public distributions.

\begin{proposition}\label{prob:mix}
Let $\mu,\nu\in\Delta(\mathcal{X})$ be distributions with $\mathrm{D}_\infty(\mu\|\nu)<\infty$. Let $\Dtil \sim \mu^n$ and $\Dhat \sim \nu^m$ be $n$ and $m$ independent samples from $\mu$ and $\nu$ respectively. Let $\Xhat$ be the support of $\Dhat$. Let $Q$ be a finite set of statistical queries $q : \mathcal{X} \to [0,1]$. Let $\alpha,\beta>0$. If $n \ge \frac{8}{\alpha^2} \log \left(\frac{4|Q|}{\beta}\right)$ and $m \ge \left(\frac{32}{\alpha^2} e^{\mathrm{D}_2(\mu\|\nu)} + \frac{8}{3\alpha} e^{\mathrm{D}_\infty(\mu\|\nu)}\right) \log \left( \frac{4|Q|+4}{\beta} \right)$, then
\[\Pr\left[ f_{\Dtil,Q}(\Xhat) \le \alpha \right] \ge 1-\beta. \]
\end{proposition}
\begin{proof}
Note that we may assume $\alpha<1$ as the result is trivial otherwise.
Let $g(x) = \mu(x)/\nu(x)$. Then $0 \le g(x) \le e^{\mathrm{D}_\infty(\mu\|\nu)}$ for all $x$ and, for $X \sim \nu$, we have $\mathbb{E}[g(X)]=1$ and $\mathbb{E}[g(X)^2] = e^{\mathrm{D}_2(\mu\|\nu)}$. Define $\omega \in \Delta(\Xhat)$ by $\omega_x = \frac{g(x)}{\sum_{x \in \Dhat} g(x)}$ for $x\in\Xhat$. Clearly $f_{\Dtil,Q}(\Xhat) \le \max_{q \in Q} \left| q(\Dtil) - \sum_{x \in \Dhat} \omega_x q(x) \right|$. 
% \gv{should the summation be over $\Xhat$?}\ts{No. We do want to incorporate the weighting of the public dataset. Perhaps there is better notation for this though?}

Fix some $q \in Q$.
By Hoeffding's inequality, \[\Pr[|q(\Dtil)-q(\mu)|\ge \alpha/4] \le 2\cdot e^{-\alpha^2n/8}.\]
For $X \sim \nu$, $\mathbb{E}[g(X)q(X)] = q(\mu)$ and $\mathsf{Var}[g(X)q(X)] \le \mathbb{E}[(g(X)q(X))^2] \le \mathbb{E}[g(X)^2] = e^{\mathrm{D}_2(\mu\|\nu)}$.
By Bernstein's inequality,
\begin{align*}
    &\Pr\left[\left|m \cdot q(\mu) - \sum_{x \in \Dhat} g(x) q(x) \right| \ge \frac{\alpha}{4} m \right] \\
    &\le 2 \cdot \exp\left(\frac{-\alpha^2 m}{32 \cdot e^{\mathrm{D}_2(\mu\|\nu)} + \frac{8}{3} \alpha \cdot e^{\mathrm{D}_\infty(\mu\|\nu)}}\right).
\end{align*}
Let $\hat m = \sum_{x \in \Dhat} g(x)$. Similarly,
\begin{align*}
    &\Pr\left[|\hat m - m| \ge \frac{\alpha}{4}m\right] = \Pr\left[\left|m - \sum_{x \in \Dhat} g(x) \right| \ge \frac{\alpha}{4}m \right] \\
    &\le 2 \cdot \exp\left(\frac{-\alpha^2 m}{32 \cdot \left(e^{\mathrm{D}_2(\mu\|\nu)}-1\right) + \frac{8}{3} \cdot \alpha \cdot e^{\mathrm{D}_\infty(\mu\|\nu)}}\right).
\end{align*}
If all three of the events above do not happen, then
\begin{align*}
    &\left| q(\Dtil) - \sum_{x \in \Dhat} \omega_x q(x) \right| = \left| \frac1n\sum_{x \in \Dtil} q(x) - \frac1{\hat m} \sum_{x \in \Dhat} g(x) q(x) \right| \\
    &\le \left| \frac1n\sum_{x \in \Dtil} q(x) - q(\mu) \right| + \left|\frac1{\hat m} \left( m q(\mu) - \sum_{x \in \Dhat} g(x) q(x) \right) \right| \\
    &+\frac{|\hat m - m|}{\hat m} |q(\mu)|
    \le \frac{\alpha}{4} + \frac{\frac{\alpha}{4} m +\frac{\alpha}{4} m}{m-\frac{\alpha}{4} m} \le \alpha.
\end{align*}
Taking a union bound over all $q \in Q$ shows that the probability that any of these events happens is at most \[2|Q|\cdot e^{\!\!-\alpha^2n/8} \!\!+\! (2|Q|\!+\!2) \cdot \exp\!\!\left(\!\frac{-\alpha^2 m}{32 \!\cdot\! e^{\mathrm{D}_2(\mu\|\nu)} \!\!+\!\! \frac{8}{3} \!\cdot\! \alpha \!\cdot\! e^{\mathrm{D}_\infty(\mu\|\nu)}}\!\!\right)\!\!,\]
which is at most $\beta$ if $n$ and $m$ are as large as the theorem requires.
\end{proof}

Having established sufficient conditions for good public data support, we bound the worst-case error of \ours running on a support $\Dsupp$. Since our method is equivalent to running \mwem on a restricted domain $\Dsupp$, its error bound will be similar to that of \mwem. \citet{HardtLM12} show that, if the number of iterations of the algorithm is chosen appropriately, then \mwem has error scaling with $\sqrt{\log(|\cX|)}$ where $\cX$ is the algorithm's data domain. Since \ours is initialized with the restricted data domain $\Xhat$ based on a public dataset of size $m$, its error increases with $\sqrt{\log |\Xhat|} \le \sqrt{\log m}$ instead. Moreover, \ours's error bound includes the best-mixture error $f_{\Dtil, \cQ}(\Xhat)$. Taken together, we present the following bound:

%The next proposition relates the accuracy of \ours\ to the size of the public dataset $m$ and the quality of the support $\Xhat$. Essentially, $\errorLBfunc_{\Dtil,Q}$ measures the error of the optimal reweighting of the support of the public dataset to match the privacy dataset.
% and the theorem below shows that \ours\ attains a reweighting that is close to optimal; the analysis mirrors that of \mwem\ \citep{HardtLM12}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Proposition
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \ts{I have edited the the statement below.}
\begin{theorem}\label{thm:acc}
% Suppose we have access to a public dataset with support $\Xhat$.
%
For any private dataset $\Dtil \in \cX^n$, set of statistical queries $Q\subset\{q:\cX\to[0,1]\}$, public dataset $\Dhat \in \cX^m$ with support $\Xhat$, and privacy parameter $\tilde{\varepsilon}>0$, \ours with parameter $T = \Theta\left( \frac{n \tilde{\eps}\sqrt{\log m}}{\log |\cQ|} + \log(1/\beta) \right)$ outputs a distribution $A$ on $\Xhat$ such that, 
with probability $\ge 1-\beta$, 
% \ts{Need to specify how to set $T$.}
\begin{align*}
    % &\max_{q\in \cQ} \abs{q(X) - q(\Dtil)} \\ 
    &\max_{q\in \cQ} \abs{q(A) - q(\Dtil)} \\
    &\leq O\pp{\sqrt{\frac{\log(|Q|) \cdot (\sqrt{\log m} +\log(\tfrac{1}{\beta})) 
   }{n\tilde{\varepsilon}}} + \errorLBfunc_{\Dtil, Q}\pp{\Dsupp}}.
       % \sqrt{\frac{\log\pp{|\Xhat| \pp{\frac{\log(|\cX|/\beta)}{m}}^{\tfrac{1}{2}}  +1 }
    % \log(Q)\log(1/\delta)\log(1/\beta)}{n\tilde{\varepsilon}}} \\ 
\end{align*}
%where $\iota =  \log(|\cQ|)\log(1/\delta)\log(1/\beta) $.%, and 
% $$\gamma_k = \sqrt{\frac{\log(2|\cX|/\beta)}{k}}$$ .
\end{theorem}


% \gv{We we have a new accuracy theorem that combines }
% \begin{theorem}
% Running \ours with parameters as in \cref{prob:mix} has error:
% \end{theorem}
% \begin{proof}
% Let $\mu$ be the best mixture corresponding to $f_{\Dtil, \cQ}(\Xhat)$. Then
% \begin{align*}
%     &\max_{q\in \cQ} \abs{q(X) - q(\Dtil)} \\\
%     &= \max_{q\in \cQ} \abs{q(X) - q(\mu) + q(\mu) - q(\Dtil)} \\ 
%     &\leq \max_{q\in \cQ} \abs{q(X) - q(\mu)} + \max_{q\in \cQ} \abs{q(\mu) - q(\Dtil)} \\
%     &\leq \max_{q\in \cQ} \abs{q(X) - q(\mu)} + \max_{q\in \cQ} \abs{q(\mu) - q(\Dtil)} \\ 
%     &\leq \max_{q\in \cQ} \abs{q(X) - q(\mu)} + f_{\Dtil, \cQ}(\cX)
% \end{align*}

% \end{proof}
%
% %%%%%%%%%%%%%%%%%%%%%%%%%
% %% Proof
% %%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}

% We use the same argument as \citet{HardtLM12} for the accuracy analysis of \mwem with the distintion that the data universe is $\Xhat$.  We use a potential argument with the KL divergence (a.k.a.~relative entropy) as the potential function:
%  \[
%  \Psi_t = \sum_{x\in \Dsupp} \Dtil(x) \log{\frac{\Dtil(x)}{A_{t}(x)}}, 
%  \]
%  where $\Dtil(x)$ denotes the relative frequency of $x$ in the dataset $\Dtil$.
%  Then they showed that the error is bounded by
%  %
%  \[
%  O\pp{
%  \sqrt{\frac{\Psi_0\log(|Q|)\log(1/\delta)}{n \tilde{\varepsilon}}}
%  }
%  \]
%  %
%  For this proof we just need to bound $\Psi_0$. First recall that
%  %
%  \begin{enumerate}
%      \item $A_0$ is the distribution over $\Xhat = \supp(\Dhat) \subset \cX$ given by $\Dhat$. Hence $A_0(x) = \Dhat(x)$ for all $x\in \Xhat$.
%      \item For any $x\in \Xhat$ $A_0(x ) \geq \tfrac{1}{m}$.
%     %  \item By assumption $|\Dtil(x) - A_0(x)| \leq \kappa$.
%  \end{enumerate}
 
 
%  Define a set of queries $Q_0\defeq \{ q_x : q_x(x') = \bbI[x' = x ] \}$. Fix $x\in \Xhat$ and  $q_x\in Q_0$, by \cref{thm:multchernoff} we have that 

% We have
% \begin{align*}
%     \Psi_0 &= \sum_{x\in \Dsupp} \Dtil(x) \log{\frac{\Dtil(x)}{A_0(x)}}  \\
%     &\leq \sum_{x\in \Dsupp} \Dtil(x) \log\pp{|\Xhat|\Dtil(x)}  \\
%     &\leq  \log{|\Xhat|} 
% \end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

% Let $\gamma(n) = \sqrt{\frac{\log(2|\cX|/\beta)}{n}}$ and $\beta>0$. Let $E_1$ be the event that $\forall_{x\in\cX}|\Dhat(x) - \nu(x)| \leq \gamma(m)$ and $E_2$ the event that $\forall_{x\in\cX}|\Dtil(x) - \mu(x)| \leq \gamma(n)$. Finally, let $E_3$ be the event that algorithm \ours\ outputs a dataset $X$ such that
% $\max_{q\in Q} \abs{q(X) - q(\Dtil)} \leq \alpha$, where
% \begin{align*}
%     \alpha =
%     \sqrt{\frac{\log\pp{|\Xhat| \kappa +1 }\log(|Q|)\log(1/\delta)\log(1/\beta)}{n\tilde{\varepsilon}}} \\ 
%     \notag
%     +\errorLBfunc\pp{\Dsupp}
% \end{align*}
% for any value of $\kappa$.


% Under event $(E_1 \cap E_2)$ we have for any $x\in\cX$:
% \begin{align*}
%     &\abs{\Dtil(x) - \Dhat(x)}  \\
%     &=\abs{\Dtil(x) - \Dhat(x) + \mu(x) - \mu(x) + \nu(x) - \nu(x) }\\
%     &\leq  |\Dtil(x) - \mu(x)| + |\Dhat(x) - \nu(x)| + |\nu(x)-\mu(x)| \\
%     &\leq \gamma(n) + \gamma(m) + \kappa_{\mu,\nu}\\ 
%     % &= \sqrt{\frac{\log(2|\cX|/\beta)}{n}} + \sqrt{\frac{\log(2|\cX|/\beta)}{m}} +  |\nu(x)-\mu(x)|\\
%     % &\leq 2 \sqrt{\frac{\log(2|\cX|/\beta)}{m}}
% \end{align*}

%  Therefore, under event $(E_1 \cap E_2 \cap E_3)$, $\Dhat $ is $\kappa$ close to $\Dtil$ with $\kappa = \gamma(n) + \gamma(m) + \kappa_{\mu,\nu}$ and we get the desired bound.
% The last step to bound the fail probability of $(E_1 \cap E_2 \cap E_3)$.
% By \cref{lem:concentration} the fail probability of $E_1$ and $E_2$ is $\beta$ and by \cref{lem:mwempuberror} the fail probability of $E_3$ is also $\beta$. Hence, by union bound on the three events we have $\pr{E_1 \cap E_2 \cap E_3} \geq 1-3\beta$, completing the proof.
% \end{proof}



% In this section, we showed that the performance of \ours depends on the best mixture error term $f_{\Dtil, \cQ}(\Xhat)$. Since $f_{\Dtil, \cQ}(\Xhat)$ is only used for the accuracy analysis,  \ours does not need to compute it. However, we might want to compute $f_{\Dtil, \cQ}(\Xhat)$ before we decide to run \ours with support $\Xhat$. Since the best mixture error $f_{\Dtil, \cQ}$, is a function that depends on the privacy data $\Dtil$, we have to release it in a privacy-preserving way. Thus the next lemma  shows that it has bounded sensitivity:
% %
% \begin{lemma}
% For any  support $S\in 2^\cX$ and set $Q$, 
% the  best mixture error function $f_{D,Q}$ is $\tfrac{1}{n}$ sensitive. 
% That is for neighboring datasets $D,D'$ : $\abs{f_{D,Q}(S)  - f_{D',Q}(S)} \leq \tfrac{1}{n}$.
% \end{lemma}
% %
% Thus, the function $f_{\Dtil, \cQ}$ is $\tfrac{1}{n}$ sensitive. It follows that we can release $f_{\Dtil, \cQ}(\Xhat)$, using the Laplace mechanism with magnitude scaled by $\tfrac{1}{n}$.


\subsection{Privacy Analysis}
The privacy analysis follows from four facts: (i) Permute-and-flip satisfies $\varepsilon_0$-differential privacy \cite{McKennaS20}, which implies $\frac12\varepsilon_0^2$-concentrated differential privacy. (ii) The Gaussian noise addition also satisfies $\frac12\varepsilon_0^2$-concentrated differential privacy. (iii) The composition property of concentrated differential privacy allows us to add up these $2T$ terms \cite{BunS16}. (iv) Finally, we can convert the concentrated differential privacy guarantee into approximate differential privacy \cite{CanonneKS20}.

\begin{theorem}
When run with privacy parameter $\tilde{\varepsilon}>0$, \ours\ satisfies $\frac12\tilde{\varepsilon}^2$-concentrated differential privacy and, for all $\delta>0$, it satisfies$\left( \varepsilon(\delta), \delta\right)$-differential privacy, where 
\begin{align*}
    \varepsilon(\delta) 
    &= \inf_{\alpha>1} \frac12\tilde{\varepsilon}^2\alpha + \frac{\log(1/\alpha\delta)}{\alpha-1} + \log(1-1/\alpha) \\
    &\le \frac12\tilde{\varepsilon}^2 + \sqrt{2\log(1/\delta)}\cdot\tilde{\varepsilon}.
\end{align*}
\end{theorem}



\endgroup




%


% The error will depend on the quality of the public dataset and the performance of the \mwem\ algorithm. Recall that, given the private dataset $\Dtil$, the error of $X\in \cX^*$ is
% \begin{align*}
%      \max_{q\in Q}\abs{q\pp{\Dtil} - q\pp{X}}
% \end{align*}

% Suppose the public dataset $\Dhat$ and the private dataset $\Dtil$ both consist of i.i.d.~draws from some distribution $\mu \in \Delta\pp{\cX}$. Then, with high probability, $\Dhat$ will approximate $\Dtil$ fairly well. To see this, fix some arbitrary query $q\in Q$. Let $m = |\Dhat|$ and $n=|\Dtil|$ be the size of the public and private datasets respectively. Both $q(\Dhat) = \tfrac{1}{m}\sum_{x\in\Dhat} q(x)$ and $q(\Dtil) = \tfrac{1}{n} \sum_{x \in \Dtil} q(x)$ have expectation $q(\mu) = \bbE_{x\sim \mu}\bb{q(x)}$ and $q(x) \in [0,1]$ is bounded for each $x \in \cX$.  By Hoeffding's inequality, \[\underset{\Dhat \sim \mu^m, \Dtil \sim \mu^n}{\Pr}\left[|q(\Dhat)-q(\Dtil)| \ge \alpha\right] \le 2 \cdot \exp\left(\frac{-2\alpha^2}{1/n+1/m}\right).\] By a union bound over all the queries $q \in Q$, if $n,m \geq \frac{\log(2|Q|/\beta)}{\alpha^2}$, then with probability at least $1-\beta$ we have $\max_{q\in Q } \abs{q(\Dtil) - q(\Dhat)} \leq \alpha$.

% One can see that if the public dataset is a large sample from the same distribution as the private data, then the problem is trivial; that is, the public data already provides a good approximation of the private data. However, this paper considers the setting where we cannot generate an arbitrarily large sample from the target distribution. In our experiments, we mainly consider two general settings. In the first, we assume that the public dataset $\Dhat$ is a sample from the target distribution $\mu$, but we have a limited small sample. \ts{Do we cover this first case?} The second scenario is that the public dataset is a large sample from a distribution different from $\mu$ (but similar enough to be useful).

% We can represent the public dataset $\Dhat$ by the tuple $(\Dsupp, \Ddist)$,
% where $\Dsupp = \supp(\Dhat)$ is the support of the public dataset 
% $\Dhat$ and $\Ddist \in \Delta(\Dsupp)$ is the distribution of $\Dhat$ over the support $\Dsupp$.


% Each dataset in $\cX^*$ can be seen as a distribution over a support. Formally, 



==> figures/acs/compare_workloads.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.6]{images/acs/compare_workloads.png}
    % \includegraphics[width=\linewidth]{images/acs/compare_workloads.png}
    \caption{Performance comparison of \ours against \hdmm on $3$-way marginals on ACS PA-18 while varying the number of workloads. We evaluate on privacy budgets $\varepsilon \in \{ 0.1, 0.25, 0.5, 1 \}$ and $\delta = \frac{1}{n^2}$ and present results of \ours using ACS PA-10 and OH-18.
    }
    \label{fig:acs_compare_workloads}
\end{figure}

==> old/figures/acs-ga/compare_benchmarks.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/acs-ga/compare_to_benchmarks.png}
    \caption{[2018 ACS, Georgia] Comparison of max error on 3-way marginals across privacy budgets $\epsilon$ where $\delta = \frac{1}{N^2}$ and the workload size is 4096. \tl{Updated. maybe combine it with PA if we keep it in the main section}
    }
    \label{fig:acs-ga_compare_benchmarks}
\end{figure}

==> old/figures/acs-pa/compare_benchmarks.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/acs-pa/compare_to_benchmarks.png}
    \caption{[2018 ACS, Pennsylvania] Comparison of max error on 3-way marginals across privacy budgets $\epsilon$ where $\delta = \frac{1}{N^2}$ and the workload size is 4096.  \tl{Updated}
    }
    \label{fig:acs-pa_compare_benchmarks}
\end{figure}

==> old/figures/acs-pa/compare_pub.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/acs-pa/compare_pub_datasets.png}
    \caption{Comparison of max errors using different public datasets to run \ours on the ACS (PA 2018), fixing $\epsilon=0.5$ and $\delta = \frac{1}{N^2}$. We evaluate on 3-way marginals at a workload size of 2048. Results for additional values of $\epsilon$ can found in Figure \ref{fig:acs-pa_compare_benchmarks_appendix}.}
    \label{fig:acs-pa_compare_pub}%
\end{figure}


==> old/figures/acs-pa/compare_pub_sizes.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/acs-pa/compare_pub_sizes.png}
    \caption{[2018 ACS, Pennsylvania] Max error on 3-way marginals while varying the fraction of the public dataset used, where $\epsilon=0.5$, $\delta = \frac{1}{N^2}$, and workload size is 4096. \tl{Updated.}}
    \label{fig:acs-pa_compare_pub_sizes}
\end{figure}

==> old/figures/acs-pa/compare_workloads.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/acs-pa/compare_workloads.png}
    \caption{[2018 ACS, Pennsylvania] Comparison of \ours (using the entire public dataset) against HDMM on 3-way marginals while varying the workload size. Results displayed are for $\epsilon=1.0$ and $\delta = \frac{1}{N^2}$. \tl{updated. What value of epsilon should we show here?}}
    \label{fig:acs-pa_compare_workloads}%
\end{figure}

==> old/figures/acs-small-pa/compare_mwem_supports.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/acs-small-pa/compare_mwem_supports.png}
    \caption{[2018 ACS (reduced), Pennsylvania] Max error on 5-way marginals across privacy budgets $\epsilon$ where $\delta = \frac{1}{N^2}$ and workload size is 3003. We run MWEM while maintaining a distribution over the domains of our public datasets (PA-10, OH-18, NJ-18) rather than the entire universe. In addition, we sample $C$ rows from the data domain and run MWEM with $C \in \{5000, 10000, 25000\}$ (labeled as MWEM (C)). \tl{Updated. Should we remove some of the MWEM+PUB so the lines aren't as crowded?}}
    \label{fig:acs-small-pa_compare_mwem_supports}%
\end{figure}


==> old/figures/acs-small-pa/compare_to_benchmarks.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/acs-small-pa/compare_to_benchmarks.png}
    \caption{[2018 ACS (reduced), Pennsylvania] Comparison of max error on 5-way marginals across privacy budgets $\epsilon$ where $\delta = \frac{1}{N^2}$. We use the maximum workload size (3003) and run \ours with the entire public dataset. \tl{updated}}
    \label{fig:acs-small-pa_compare_to_benchmarks}%
\end{figure}


==> old/figures/acs-small-pa/improvement_over_unif.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/acs-small-pa/improvement_over_unif.png}
    \caption{Difference in max error (\textbf{higher} is better) of \ours vs. \mwem initialized with a uniform distribution over the public data domain. Experiments are run across privacy budgets $\epsilon$ where $\delta = \frac{1}{N^2}$. We evaluate over 5-marginal queries at the maximum workload size of 3003. \tl{Updated.}}
    \label{fig:acs-small-pa_improvement_over_unif}%
\end{figure}


==> old/figures/adult/compare_to_benchmarks.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/adult/compare_to_benchmarks.png}
    \caption{Max error on 3-way marginals across privacy budgets $\epsilon$ where $\delta = \frac{1}{N^2}$ and the workload size is 256. When running \ours, each public dataset is created by sampling from the public partition with some bias $\Delta$ over the attributes \textit{sex} (labeled as MWEM+PUB ($\Delta$)).}
    % \label{fig:adult_compare_to_benchmarks}%
\end{figure}

==> old/tables/acs-pa/compare_pub_init.tex <==
\begin{table}
    \begin{center}
    \begin{tabular}{lc}
        \toprule
        Public Dataset & Initial Error \\
        \midrule
        PA (2010) & $0.0967$ \\
        OH (2018) & $0.1370$ \\
        MI (2018) & $0.1653$ \\
        IL (2018) & $0.1599$ \\
        NJ (2018) & $0.3389$ \\
        \bottomrule
    \end{tabular}
    \end{center}
\caption{Table comparing the initial error of each public dataset ($\epsilon = 0$).}
\label{tab:compare_init_errors}
\end{table}

==> tables/acs/runtime_-_other.tex <==
\begin{table}[!h]
\centering
\caption{Per iteration run-time comparison (averaged over $T=100$ iterations) between \ours and \mwem on 3-way marginals over 2018 ACS (reduced)-PA, varying the workload size. \ours uses PA-18 as its public dataset.}
\setlength\tabcolsep{9pt}
\begin{tabular}{l c c c c c c }
    \toprule
    & \multicolumn{4}{c}{\textsc{Workload Size}} \\
    \textsc{Algo}. & $512$ & $1024$ & $2048$ & $3003$ \\
    \midrule
    \ours & $0.0209$ & $0.0439$ & $0.1099$ & $0.1847$ \\
    \mwem & $0.1527$ & $0.3046$ & $0.6138$ & $0.9193$ \\
    \hdmm & $4.0775$ & $8.2583$ & $16.3315$ & $23.8415$ \\
    \bottomrule
\end{tabular}
\label{tab:acs_small_runtime}
\end{table}

==> tables/acs/runtime__old_with_hdmm_.tex <==
\begin{table}[!t]
\centering
\caption{Run-time comparison between \ours and \mwem on the 2018 ACS PA and ACS (reduced) PA, denoted as \textsc{Full} and \text{Red.} respectively. We compare the per-iteration and total run-time time between \ours (using PA-10 as the public dataset) and \mwem. We express the total run-time of \ours and \mwem in terms of the hyperparameter $T$, which determines the number of iterations we run each algorithm for. Experiments are conducted using a single core on a i5-4690K CPU (3.50GHz) machine.}
\setlength\tabcolsep{9pt}
\begin{tabular}{l l c c}
    \toprule
    & & \multicolumn{2}{c}{\textsc{Time (seconds)}} \\
    & \textsc{Algo}. & \textsc{Per-iter.} & \textsc{Total} \\
    \midrule
    \multirow{2}{*}{\textsc{Red.}}
    & \ours & $0.185$ & $0.185 \times T$ \\
    & \mwem & $0.919$ & $0.919 \times T$ \\
    % & \hdmm & $-$ & $23.841$ \\
    \midrule
    \multirow{2}{*}{\textsc{Full}}
    & \ours & $2.021$ & $2.021 \times T$  \\
    & \mwem & $-$ & $-$ \\
    % & \hdmm & $-$ & $24.236$ \\
    \bottomrule
\end{tabular}
\label{tab:acs_small_runtime}
\end{table}
